PinnerSage: Multi-Modal User Embedding Framework for Recommendations at Pinterest

Latent user representations are widely adopted in the tech industry for powering personalized recommender systems. Most prior work infers a single high dimensional embedding to represent a user, which is a good starting point but falls short in delivering a full understanding of the user's interests. In this work, we introduce PinnerSage, an end-to-end recommender system that represents each user via multi-modal embeddings and leverages this rich representation of users to provides high quality personalized recommendations. PinnerSage achieves this by clustering users' actions into conceptually coherent clusters with the help of a hierarchical clustering method (Ward) and summarizes the clusters via representative pins (Medoids) for efficiency and interpretability. PinnerSage is deployed in production at Pinterest and we outline the several design decisions that makes it run seamlessly at a very large scale. We conduct several offline and online A/B experiments to show that our method significantly outperforms single embedding methods.

==> sections/background.tex <==

\subsection{Pinterest Overview}
% yzhou: moving image to Intro, and replaced with a wider one screenshot on desktop
% \begin{figure}[h]
% \caption{Pinterest Homefeed}
% \label{fig:pinterest}
% \centering
% \includegraphics[scale=0.17]{images/pinterest.jpg} \\
% \end{figure}

Recommender systems at Pinterest follow a classic two-stage process: candidate generation and candidate ranking. This architecture is commonly used in the industry. Multiple candidate sources can be developed and iterated independently without interference, maximizing collaboration efficiency within large groups. At candidate retrieval stage, recall and retrieval scale are both emphasized to achieve high candidate coverage; while at ranking stage, more expensive model computation is afforded to deliver the final best recommendations. Embedding-based user representation is able to provide a unique candidate retrieval pool, differing from topics matching or graph-based traversal \cite{pixie}; and to allow embeddings directly digested as features in the ranking stage.

\subsection{Challenges}
Unique challenges are encountered during system development:

\textbf{Drawbacks of Single Embedding.} As demonstrated in Figure \ref{fig:curse_of_single_embedding}, embedding space with high dimension usually cannot guarantee the transitive similarity of a linear combination of embedding items. When, for example, a user's interests: painting, shoe and sci-fi being projected into three spots of a high dimensional space; the average point can be an irrelevant new interest, even when the close neighbors of each interest are highly relevant. As long as similarity is still measured via space distance, this issue cannot be bypassed since any embedding can be expressed as a linear combination of Eigen vectors of the space. Therefore, when forcing a user's interest be represented as a single embedding, it becomes a dilemma that we either land in the middle, delivering irrelevant random outcome; or land too close, generating results biased towards one particular interest. 
\label{ref:section_curse_of_single_embedding}
\begin{figure}[t]
\centering
\includegraphics[scale=0.25]{images/curse_of_single_embedding.png} \\
\caption{Averaging in Embedding Space}
\label{fig:curse_of_single_embedding}
\end{figure}

\textbf{Diverse User Action Sequence.} As shown in Figure \ref{fig:activities}, typical users on Pinterest engages with a diverse range of topics. Within the same session, a user can focus on a specific topic or engage with multiple topics periodically. A good embedding model, therefore needs to encode rich diversity of the user behavior, or it may miss out parts of user interests.


% \textbf{Customization v.s. Unification:} Most embedding models require a wide coverage of features with specific objective functions trained towards a narrow problem. Such customization becomes expensive and hard to manage if user embeddings customization is needed for each individual application. For example, it is hard to decide the boundary based on whether or not a user embedding representation should encode co-engagement, text signal, visual signal and to what degree. As a result, we purposefully seek to find a unified common representation of users, that does not subject to specific use cases or specific objective to simplify overall architecture. 

% NOTE: Commented out, was also discussed in method
% \subsection{Motivation}
% Under circumstances discussed above, PinnerSage intentionally derives multi-model embedding representation in the same space of pin embeddings to gain several benefits: 1) Better representing diverse user interests; 2) enabling direct similarity measurement between user and pins; 3) providing a consistent unified model built for both user and item embeddings compatible with multiple application cases; 4) yielding higher cost efficiency by having a shared embedding serving infrastructure. These setups are treated as presumptions, and methods and experiments are developed and carried out under such constraints. 

